A Year of the DSA Transparency Database: What it (Does Not) Reveal About Platform Moderation During the 2024 European Parliament Election

Social media platforms face heightened risks during major political events; yet, how platforms adapt their moderation practices in response remains unclear. The Digital Services Act Transparency Database offers an unprecedented opportunity to systematically study content moderation at scale, enabling researchers and policymakers to assess platforms' compliance and effectiveness. Herein, we analyze 1.58 billion self-reported moderation actions taken by eight large social media platforms during an extended period of eight months surrounding the 2024 European Parliament elections. Our findings reveal a lack of adaptation in moderation strategies, as platforms did not exhibit significant changes in their enforcement behaviors surrounding the elections. This raises concerns about whether platforms adapted their moderation practices at all, or if structural limitations of the database concealed possible adjustments. Moreover, we found that noted transparency and accountability issues persist nearly a year after initial concerns were raised. These results highlight the limitations of current self-regulatory approaches and underscore the need for stronger enforcement and data access mechanisms to ensure that online platforms uphold their responsibility in safeguarding democratic processes.

==> tables/info-columns.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \renewcommand{\arraystretch}{1.2}
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{p{0.20\textwidth}p{0.30\textwidth}p{0.5\textwidth}}
        \toprule
        \textbf{field} & \textbf{reference} & \textbf{description} \\
        \midrule
        \texttt{application date} & \S 4.1 Application Date & Indicates when a content moderation decision was applied \\
        \midrule
        \texttt{automated decision} & \S10. Automated Decision & Indicates whether the decision to moderate a content was automatic or not \\
        \midrule
        \texttt{automated detection} & \S9. Automated Detection & Indicates whether moderated content was detected automatically or not \\
        \midrule
        \texttt{category} & \S16. CATEGORY \& SPECIFICATION & Indicates the type of illegality or incompatibility with the platform's terms of services that led to a content being moderated \\
        \midrule
        \texttt{content date} & \S2.3. Date on which the content was created on the online platform & Indicates when moderated content was created \\
        \midrule
        \texttt{content type} & \S 2.1. Type of content affected & Type of the moderated content (e.g. audio, video, image, etc.) \\
        \midrule
        \texttt{content type other} & \S2.2. Specification of Content Type ``Other'' & Specification required when content type is ``other'' \\
        \midrule
        \texttt{decision ground} & \S11. Decision Grounds & Indicates whether the moderated content was deemed allegedly illegal or incompatible with the platform’s terms of service \\
        \midrule
        \texttt{incompatible content illegal} & \S12.2. Explanation of the applicability of the legal ground & Explains why a specific content has been deemed illegal according to Article 17(3)(d) of DSA \\
        \midrule
        \texttt{incompatible content ground} & \S13.1. Incompatible Content Grounds & Explains why a specific content has been deemed incompatible with the platform's terms of service \\
        \bottomrule
    \end{tabular}}
    \caption{Complete list of the DSA Transparency Database (\texttt{DSA-TDB}) fields analyzed in this study. For each field, we report its name, reference to the official documentation, and brief description.}
    \label{tab:dsa-fields}
\end{table*}

